A Frequency Domain Analysis of Slow Coherency in Networked Systems

Network coherence generally refers to the emergence of simple aggregated dynamical behaviours, despite heterogeneity in the dynamics of the subsystems that constitute the network. In this paper, we develop a general frequency domain framework to analyze and quantify the level of network coherence that a system exhibits by relating coherence with a low-rank property of the system's input-output response. More precisely, for a networked system with linear dynamics and coupling, we show that, as the network's \emph{effective algebraic connectivity} grows, the system transfer matrix converges to a rank-one transfer matrix representing the coherent behavior. Interestingly, the non-zero eigenvalue of such a rank-one matrix is given by the harmonic mean of individual nodal dynamics, and we refer to it as the coherent dynamics. Our analysis unveils the frequency-dependent nature of coherence and a non-trivial interplay between dynamics and network topology. We further show that many networked systems can exhibit similar coherent behavior by establishing a concentration result in a setting with randomly chosen individual nodal dynamics.

==> Review/R8_231507.tex <==
This submission develops a general framework to analyze and quantify the level of network coherence that a system exhibits by relating coherence with a low-rank property of the system. For a networked system with linear dynamics and coupling, authors show that, as the network connectivity grows, the system transfer matrix converges to a rank-one transfer matrix representing the coherent behavior. The analysis in this paper unveils the frequency dependent
nature of coherence and a non-trivial interplay between dynamics and network topology. Authors further show that many networked systems can exhibit similar coherent behavior by establishing a concentration result in a setting with randomly chosen individual nodal dynamics.

The research motivation is well presented, and it is a great advantage in that complete proof is well presented. However, there are too few figures in the paper, especially in the first few pages. More descriptive pictures should be supplemented to show the relationship of the analysis. For example, a figure about the overall framework is necessary, in which the pointwise coherence and uniform coherence are linked by some relationship. Moreover, please
explain “point-wise convergence”.

The difficulty from homogeneous node dynamics to heterogeneous nodal dynamics should
be clarified again. For example, let g_i(s)=\Delta_i \bar{g}(s), where \Delta_i can be separated fromg g_i(s) to
get similar results. The following results look easy to obtain. So, the contributions should be
clarified again.

==> old_intro.tex <==
Coordinated behavior in network systems has been a popular subject of research in many fields, including physics~\cite{Bressloff1999}, chemistry~\cite{Kiss2002}, social sciences~\cite{DeGroot1974}, and biology~\cite{Mirollo1990}. Within engineering, coordination is essential for the proper operation of many networked systems including power networks~\cite{jpm2017cdc,Paganini2019tac}, data and sensor networks~\cite{mmhzt2015ton,m2014phd-thesis}, and autonomous transportation~\cite{Sepulchre2008706,Olfati-Saber2007,Jadbabaie2003988,Bamieh2012}.
While there exist many expressions of this behavior, two forms of coordination have particularly received thorough attention by the control community: Consensus and synchronization.

Consensus~\cite{DeGroot1974, Olfati-Saber2007, Jadbabaie2003988, Bamieh2012, Tegling19,Olfati-Saber20041520, Ghaedsharaf2019}, on one hand, refers to the ability of the network nodes to asymptotically reach a common value over some quantities of interest.
Many extensions of this problem include the study of robustness and performance of consensus networks in the presence of noise~\cite{Jadbabaie2003988,Bamieh2012,Tegling19}, time-delay~\cite{Olfati-Saber20041520, Ghaedsharaf2019}, and switching graph topology~\cite{Ghaedsharaf2019}.
Synchronization~\cite{Mirollo1990,mmhzt2015ton,m2014phd-thesis,Sepulchre2008706,Nair2008661,Kim2011200,Wieland2011}, on the other hand, refers to the ability of network nodes to follow a commonly defined trajectory. Although for nonlinear systems synchronization is a structurally stable phenomenon, in the linear case~\cite{Nair2008661, Sepulchre2008706, Kim2011200, Wieland2011}, synchronization requires the existence of a common internal model that acts as a virtual leader~\cite{Kim2011200,Wieland2011}.

A closely related notion of coordination emerges when looking at how the network agents collectively respond to disturbances. In this setting, agents with noticeably different input-output responses, can present a similar, i.e., coherent, response when interconnected.
% Generally, without nonlinearity, this coordinated behavior relies on the coherence among all nodes. 
% Coherence mainly depends on the strength of the network coupling and 
A vast body of work, triggered by the seminal paper~\cite{Bamieh2012}, has quantitatively studied the role of the network topology in the emergence of coherence. Examples include, directed~\cite{Tegling19} and undirected~\cite{Oral17} consensus networks, transportation networks~\cite{Bamieh2012}, and power networks~\cite{Paganini2019tac,Bamieh2013,Andreasson17,psf17cdc}. 
% There has been a large amount of work on formalizing such relation for different networks such as consensus networks~\cite{Bamieh2012,Tegling19}, transportation networks~\cite{Bamieh2012}, and power networks~\cite{Paganini2019tac,Andreasson17}. 
% Also, the coherence of networks over digraph is discussed in~\cite{Oral17}. 
The key technical approach amounts to quantify the level of coherence by computing the $\mathcal{H}_2$-norm of the system for appropriately defined nodal disturbance and performance signals. Broadly speaking, the analysis shows a reciprocal dependence between the performance metrics and the non-zero eigenvalues of the network graph Laplacian, validating the fact that strong network coherence (low $\mathcal{H}_2$-norm) results from the high connectivity of the network (large Laplacian eigenvalues).
% In particular, coherence in the $\mathcal{H}_2$ sense can be characterized by the sum of all reciprocal of the non-zero eigenvalues of graph Laplacian for undirected graph, which also motivates graph topology design\cite{Summers15} to increase network coherence. 
Unfortunately, the analysis strongly relies on a homogeneity~\cite{Bamieh2012,Tegling19, Oral17,Bamieh2013, Andreasson17,psf17cdc} or proportionality~\cite{Paganini2019tac} assumption of the nodal transfer functions, and thus fails to characterize how individual heterogeneous node dynamics affect the overall coherent network response.

% dynamics, and the node dynamics are usually simple: integrator or first-order dynamics. It remains unknown, how the strong network coupling would affect the behavior of general networks, which most likely are heterogeneous with complex node dynamics.  
In this paper, we seek to overcome these limitations by formalizing network coherence by the presence of a low-rank structure, of the system transfer matrix, that appears when the network feedback gain is high. 
% In this paper, we seek to overcome these limitations by formalizing the emergence of network coherence as the convergence of the network transfer matrix in the frequency domain to a low-rank from.
More precisely, we show that for linear network systems, as the network's effective algebraic connectivity (a frequency-dependent notion to be later defined) grows, the system transfer matrix converges to a rank-one transfer matrix with identical element-wise transfer functions. Interestingly, this transfer function is given by the harmonic mean of individual nodal dynamics, which we refer to as coherent dynamics.  In addition, we provide the concentration result of such coherent dynamics in large-scale stochastic networks where the node dynamics are given by random transfer functions. Furthermore, we utilize our frequency-domain results to formally show the coherent response in time domain of the network subject to certain classes of input signals.

% This frequency domain analysis provides a deeper characterization of relationship between coherent behavior and network connectivity, and furhter suggests that we can characterize the exact coherent behavior according to the individual node dynamics, or, in the stochastic setting, the probabilistic distribution of node dynamics. Here tightly-connected networks refer to networks with large algebraic connectivity.

This frequency domain analysis provides a deeper characterization of the role of both, network topology and node dynamics, on the coherent behavior of the network. In particular, our results make substantial contributions towards the understanding of coordinated and coherent behavior of network systems in many ways:
\begin{itemize}
    \item We present a general framework in frequency domain to analyze the coherence of heterogeneous networks. We show that network coherence emerges as a low rank structure of the system transfer matrix as we increase the effective algebraic connectivity--a frequency-varying quantity that depends on the network coupling strength and  dynamics.
    \item Unlike previous works, our analysis applies to networks with  heterogeneous nodal dynamics, and further provides an explicit characterization in the frequency domain of the coherent response to disturbances. Thus, in this way, our results highlight the contribution of individual nodal dynamics to the network's coherent behavior.
    \item The analysis further suggests that network coherence is a frequency-dependent phenomenon. That is, the ability for nodes to respond coherently depends on the frequency composition of the input disturbance. {\ifthenelse{\boolean{color}}{\color{blue}}{} We further explicitly connect our frequency domain analysis to time domain notions of coherence.}
    \item By providing an exact characterization of network's coherent dynamics, our analysis can be further applied in settings where only distributional information of the netwok composition is known. More precisely, we show that the coherent dynamics of tightly-connected networks with possibly random nodal dynamics are well approximated by a deterministic transfer function that only depends on the statistical distribution of node dynamics. 
    % \item Our analysis also leads to a general methodology to accurately aggregate coherent nodes. In particular, for power networks, our results theoretically demonstrate the difficulty of aggregating synchronous generators with heterogeneous turbine dynamics.
\end{itemize}

{\ifthenelse{\boolean{color}}{\color{blue}}{}Prior works on coherence primarily study homogeneous networks~\cite{Bamieh2012,Andreasson17,psf17cdc} and proportional networks~\cite{Paganini2019tac}, where the network can be diagonalized into $n$ individual dynamics,  each corresponding to one eigenvalue of the network Laplacian. However, such techniques to study coherence cannot be generalized to non-proportional heterogeneous networks. In fact, in such setting, it is a priori unclear what a good representation of the coherent response is. Our new frequency domain framework allows one to analyze coherence in general heterogeneous networks.

Notably, the problem of characterizing coherent dynamics is unique to heterogeneous networks, since the coherent dynamics for homogeneous networks are exactly equal to the common nodal dynamics. In real applications, however,  such as power networks, such characterization is relevant to model reduction~\cite{Germond1978,Apostolopoulou2016,Guggilam2018} and control design~\cite{jbvm2021lcss}. Our analysis provides, in the asymptotic sense, the exact characterization of coherent dynamics that can be used in control design for heterogeneous networks.
}

